FastMoE: A Fast Mixture-of-Expert Training System

Mixture-of-Expert (MoE) presents a strong potential in enlarging the size of language model to trillions of parameters. However, training trillion-scale MoE requires algorithm and system co-design for a well-tuned high performance distributed training system. Unfortunately, the only existing platform that meets the requirements strongly depends on Google's hardware (TPU) and software (Mesh Tensorflow) stack, and is not open and available to the public, especially GPU and PyTorch communities. In this paper, we present FastMoE, a distributed MoE training system based on PyTorch with common accelerators. The system provides a hierarchical interface for both flexible model design and easy adaption to different applications, such as Transformer-XL and Megatron-LM. Different from direct implementation of MoE models using PyTorch, the training speed is highly optimized in FastMoE by sophisticated high-performance acceleration skills. The system supports placing different experts on multiple GPUs across multiple nodes, enabling enlarging the number of experts linearly against the number of GPUs. The source of FastMoE is available at https://github.com/laekov/fastmoe under Apache-2 license.

==> 11unused.tex <==
Feed forward network is one of the most import components in the transformer model, which is basic building block of other large models.
A feed forward network contains two linear layers $L_1, L_2$ and an activation function $F_a$.
The input to the feed forward network is a 2d tensor $x_i$ of size $b \times d$, where $b$ stands for batch size, and $d$ is the dimension of features. 
The output of the network is a tensor with similar size to the input tensor.
The computation is shown in algorithm \ref{algo:ffn}.

\begin{algorithm}[ht]
% \small
    \caption{Forward computation of a feed forward network}
    \label{algo:ffn}
    \begin{algorithmic}[1]
    \Require{Linear layers $L_1, L_2$}
    \Require{Activation function $F_a$}
    \Function {FFN}{$x_i$}
        \State $x_h \Leftarrow L_1(x_i)$
        \State $x_a \Leftarrow F_a(x_h)$
        \State $x_o \Leftarrow L_2(x_a)$
        \State \Return $x_o$
    \EndFunction
    \end{algorithmic}
\end{algorithm}

A commonly used activation function $F_a$ is $ReLU$, which is defined as follow.

$$ReLU(x) = \begin{cases}
x & x \geq 0 \\
0 & x < 0
\end{cases}$$

If the input of the $ReLU$ operator is uniformly distributed around $0$, the output of the operator will be $50\%$ sparse.
However, an important observation is that in a well-trained network, the output of the activation, $x_a$ in our algorithm, can contain less than $3\%$ non-zero elements.
This is due to the sparsity of the language, each word, or token, are specifically assigned to some certain meaning.

An intuitive optimization potential is whether sparse BLAS operator, such as \texttt{SpMM} can be directly used to perform $L_2$, instead of \texttt{GeMM},
but this approach is proved to be useless.
\texttt{SpMM} operators are specially optimized on sparse storage formats like CSR, but $x_h$ is the output of a \texttt{GeMM} operator, which is stored in dense format.
Additionally, note that equal amount of computation is needed to perform $L_1$ and $L_2$.
Even if perfect fusion is applied on $L_1, F_a, L_2$, only zero computation of $L_2$ can be removed. 
The speed up of training or inference cannot be more than $2\times$.


==> 20ack.tex <==
Maybe we need to mention BAAI here?
